Non-invasive and noise-robust light focusing using confocal wavefront shaping

Wavefront-shaping is a promising approach for imaging fluorescent targets deep inside scattering tissue despite strong aberrations. It enables focusing an incoming illumination into a single spot inside tissue, as well as correcting the outgoing light scattered from the tissue, by modulating the incoming and/or outgoing wavefronts. Previously, wavefront shaping modulations have been successively estimated using feedback from strong fluorescent beads, which have been manually added to a sample. However, ideally, such feedback should be provided by the fluorescent components of the tissue itself, whose emission is orders of magnitude weaker than the one provided by beads. When a low number of photons is spread over multiple sensor pixels, the image is highly susceptible to noise, and the feedback signal required for previous algorithms cannot be detected. In this work, we suggest a wavefront shaping approach that works with a confocal modulation of both the illumination and imaging arms. Since the aberrations are corrected in the optics before the detector, the low photon budget can be directed into a single sensor spot and detected with high SNR. We derive a score function for modulation evaluation from mathematical principles, and successfully use it to image EGFP labeled neurons, despite scattering through thick tissue.

==> tex_files/fig_SNR_2.tex <==
\begin{figure*}[t!]
	\begin{center}
		
		\begin{tabular}{@{}c@{~~}c@{~~}c@{~~}c@{}}
			


			\includegraphics[width= 0.2\textwidth]{figs/fig_SNR2/1.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_SNR2/2.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_SNR2/3.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_SNR2/5.png}\\
			SNR = 725&SNR = 855&SNR = 1443&SNR = 3032
			
			
		\end{tabular}
		\captionof{figure}
				{}
		\label{fig:fig_SNR_2}
	\end{center}
\end{figure*}


==> tex_files/fig_big_area_chicken.tex <==
\begin{figure*}[t!]
	\begin{center}

		\begin{tabular}{@{}c@{~~}c@{~~}c@{}}

			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_06_05_15_57_55/1.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_06_05_15_57_55/2.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_06_05_15_57_55/3.png}\\
			
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_06_08_18_48_03/1.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_06_08_18_48_03/2_arrow.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_06_08_18_48_03/3.png}\\
			(a) Uncorrected  & (b) Corrected & (c) Reference\\
			 Main Camera &  Main Camera &  Validation Camera\\
			
			
		\end{tabular}
		\caption{Imaging a wide area through chicken breast tissue: (a) image of the neuron from the main camera with no correction, strong scattering is present and the neuron structure is lost. (b) Image with our modulation correction, the neuron shape as well as some of the axons are revealed. (c) A  reference  image of the same neuron, from the validation camera. The arrow marks a spot at which  optimization has converged. This spot is darker as it bleached during optimization.  
		}\label{fig:big_area}
	\end{center}
\end{figure*}


==> tex_files/fig_big_area_parafilm.tex <==
\begin{figure*}[t!]
	\begin{center}

		\begin{tabular}{@{}c@{~~}c@{~~}c@{~~}c@{}}
			
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_05_16_17_21_45/1.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_05_16_17_21_45/conf.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_05_16_17_21_45/2_arrow.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_05_16_17_21_45/3.png}\\			
			
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_04_30_16_12_12/1.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_04_30_16_12_12/conf.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_04_30_16_12_12/2.png}&
			\includegraphics[width= 0.2\textwidth]{figs/fig_big_area/2023_04_30_16_12_12/3.png}\\			
			(a) Uncorrected  &(b) Confocal& (c) Corrected & (d) Reference \\ 
			Main Camera  &Main Camera     & Main Camera   & Validation Camera \\
		\end{tabular}
%		\caption
		\captionof{figure}
		{Imaging a wide area through parafilm: (a) Image of the neuron from the main camera with no correction, strong scattering is present and the neuron structure is lost. (b) A confocal scan image of the target is also aberrated. (c) Image with our modulation correction, the neuron shape as well as some of the axons are revealed. (d) A  reference  image of the same neuron, from the validation camera. The arrow marks a spot at which  optimization has converged. This spot is darker as it bleached during optimization.  %In this figure, the   scattering layer is parafilm.
		 }\label{fig:big_area_parafilm}
	\end{center}
\end{figure*}


==> tex_files/fig_setup_simp_2.tex <==
\begin{figure*}[t!]
	\begin{center}
		\begin{tabular}{@{}c@{~}c@{}}
			\includegraphics[width= 0.5\textwidth]{figs/System/system_simp_2_mod.png}
			\includegraphics[width= 0.5\textwidth]{figs/System/system_simp_2_no_mod.png}
		\end{tabular}
	\end{center}
	\caption{}\label{fig:setup_simp_2}
\end{figure*}



==> tex_files/metrics_long.tex <==

\section{Scoring wavefront-shaping modulations}
\label{sec:metrics}
To estimate  a wavefront shaping modulation we first need   a score function %\IK{as mentioned: ``metric" is much better - I'll let you decide and change everywhere (alternatively, maybe ``objective function" instead of ``score function", but it is something else)} 
that can evaluate the focusing quality facilitated by a candidate modulation mask, using a noninvasive feedback alone. We start by reviewing scores that were previously introduced in the literature and then propose our new, noise-robust confocal score. 


\boldstart{Image quality scores:}
Modulation evaluation is a simpler task when the same modulation can correct a sufficiently large isoplanatic image region. This assumption was made by 
 adaptive optics research~\cite{Booth2014,Ji2017review,HampsonBooth21review,Bonora:13,Antonello:20} and also by  wavefront shaping approaches~\cite{YeminyKatz2021,Stern:19,Daniel:19}.
When  the same modulation can correct a large image region, one often evaluates the quality of the resulting image, either in terms of contrast~\cite{Ji2017review},  sharpness, or variance~\cite{YeminyKatz2021}. 
However, for thick tissue, wavefront shaping correction can vary quickly between nearby pixels,  and a modulation may only explain a very local region.  This case makes the above image quality scores less applicable, as inherently they evaluate the quality of an image region rather then a pixel. For spatially varying modulations, ideally, we would like to be able to  evaluate the success of the modulation based on a per-pixel criteria. 

%\IK{I commented a full paragraph that you wrote twice...}
%\boldstart{The total intensity score:}
%Consider  a configuration where we only try to correct the illumination arm, and the SLM in the imaging arm of \figref{fig:setup} is not used (equivalently, $ \DiagM(\CamSLMVect)$ in \equref{eq:img-form-coherent} \IK{!} is the identity matrix). The easiest score function that was considered in the literature~\cite{Katz:14,Ji2017review} is just the total intensity measured over   the entire sensor plane. 
%Using \equpref{eq:img-form-incoherent} {eq:bounded-rows} it is easy to show that this total intensity score reduces to \vspace{-0.1cm}
%\BE\label{eq:metric-TI}
%\Mtric_{\text{TI}}(\bu)\equiv\sum_x I(x)=\sum_k |\bou_k|^{2\alpha}.
%\vspace{-0.1cm}\EE
%Since   the energy at the target  is bounded (see \equref{eq:bounded-v}),
%for the case $\alpha>1$ this score is maximized when $\bou$ is a one-hot vector, which equals $1$ at a single entry and $0$ at all the others. 
%Therefore, in two-photon fluorescence finding a good modulation is easy. If we manage to modulate the illumination such that it focuses all the excitation energy in a single spot, the emitted power is maximized. 
%
%Two-photon fluorescence is however more expensive and harder to implement, and solutions that can use a single-photon excitation feedback are  highly desired. However, in the single photon case where $\alpha=1$, \equref{eq:metric-TI} reduces to the total power in $\bou$, $\Mtric_{\text{TI}}(\bu)= \sum_k |\bou_k|^{2}$ and since this power is fixed, the same amount of energy returns whether we spread the excitation power over multiple fluorescence sources or bring all of it into one spot. 
%Therefore, wavefront shaping using single-photon fluorescence has remained an open challenge in the literature until recently. 

\boldstart{The total intensity score:}
Consider  a configuration where we only try to correct the illumination arm, and the SLM in the imaging arm of \figref{fig:setup} is not used (equivalently, $ \DiagM(\CamSLMVect)$ in \equref{eq:img-form-incoherent} is the identity matrix). The simplest score that was considered in the literature~\cite{Katz:14,Ji2017review} is just the total intensity measured over   the entire sensor plane. 
Using \equpref{eq:img-form-incoherent} {eq:bounded-rows} it is easy to show that this total intensity score reduces to \vspace{-0.1cm}
\BE\label{eq:metric-TI}
\Mtric_{\text{TI}}(\bu)\equiv\sum_x I(x)=\sum_k |\bou_k|^{2\alpha}.
\vspace{-0.1cm}\EE
Since   the energy at the target  is bounded (see \equref{eq:bounded-v}),
for the case $\alpha>1$ this score is maximized when $\bou$ is a one-hot vector, which equals 1 at a single entry and zero at all the others. 
Therefore, in two-photon fluorescence finding a good modulation is well-defined. If we manage to modulate the illumination such that it focuses all the excitation energy in a single spot, the emitted power is maximized. 

Two-photon fluorescence is  expensive and hard to implement, and solutions that can use a single-photon excitation feedback are  highly desired. However, in the single-photon case where $\alpha=1$, \equref{eq:metric-TI} reduces to the total power in $\bou$, $\Mtric_{\text{TI}}(\bu)= \sum_k |\bou_k|^{2}$, and since this power is fixed, the same amount of energy returns whether we spread the excitation power over multiple fluorescence sources or bring all of it into one spot. 
Therefore, wavefront shaping using single-photon fluorescence has remained an open challenge in the literature until recently. 

\boldstart{The variance maximization score:}
Following on a setup that modulates only the illumination and not the imaging arm, 
Boniface \etal~\cite{Boniface:19} have recently suggested that to evaluate focusing with linear single-photon feedback, one should  maximize the variance of the intensity measured by the sensor. The idea is that if we manage to focus all the excitation light at a single spot, the emitted light scattered through the tissue will generate a highly varying speckle pattern on the sensor plane. If the excitation is not focused, multiple sources emit simultaneously. The light emitted by these sources sums incoherently,  and hence the variance of the speckle pattern on the sensor decays. 
A short calculation shows %\IK{I put the equation font as small because it was too large, feel free to revert; another option is to use 2 lines}
\vspace{-0.3cm}
\BEA %\vspace{-0.1cm} 
	\Mtric_{\text{Var}}(\bu)\!&\!\equiv\!& \!{\text{Var}}[I]\equiv\frac1{n}\sum_x |I(x)|^2 -\left(\frac1{n}\sum_x I(x)\right)^2 \nonumber
	\\
	\!&\!\propto\!&\! \sum_k |\bou_k|^4,
\vspace{-0.1cm}
\EEA
 where $n$ is the number of image pixels.
Hence, as before, the score is a non-linear function of the power at different fluorescent particles and is maximized by a one-hot vector. 
\input{./tex_files/fig_data_type}

This score is an important advance; however, it is hard to evaluate for low SNR biological sources.
%This score is an important advance of the state-of-the-art,
%. In practice the method was demonstrated on fluorescent beads and not on real  biological subjects.
%The main difference between beads and real subjects were 
%but it may be hard to evaluate it with sufficient noise robustness using weak biological sources. 
To demonstrate this, \figref{fig:data_type} visualizes two types of fluorescent emissions,   when excitation light is correctly focused into a single spot.  \figref{fig:data_type}(a) demonstrates an invitrogen bead (ThermoFisher Fluo-Spheres dark red) that was  attached to a scattering layer. This is a strong source, and a clear speckle pattern is imaged. The authors of~\cite{Boniface:19} have demonstrated their approach on similar beads. However, biological samples are often significantly weaker than  such beads. For example, in \figref{fig:data_type}(c) we image EGFP neurons sliced out of  a mouse brain. The fluorescent emission here is orders of magnitudes weaker. One can see that rather than  a real speckle pattern, we mostly image noise. 
The variance of this image is dominated by the noise variance rather than the actual speckle variance.
While one can reduce imaging noise by using a longer exposure or by increasing the power of the excitation laser, the optimization of~\cite{Boniface:19} requires capturing many images of the same target, and usually the neuron  bleaches well before  convergence. 
%Evaluating the variance of this image may end up with the noise variance rather than the speckle variance. 
%   From this noisy emission the variance metric cannot be successfully evaluated.  



\boldstart{Confocal energy score:}
In this research we suggest a new score for evaluating a wavefront shaping modulation. While the previous score corrected only the illumination arm, inspired by~\cite{Booth2002,Choi2015}, we suggest to correct both arms, using two modulations denoted by $\binu,\boutu$.
 As emission is very weak,  the fact that the SLM correction is applied before imaging helps collect all photons at one sensor pixel and improve SNR. 
% put the same correction at both illumination and imaging arms. 
%The idea is that if we find a modulation focusing all excitation light into one spot, due to reciprocity, the same modulation  also corrects the emitted light,  bringing all of it into a single sensor pixel (assuming the excitation and emission wavelengths are sufficiently similar). 
To score the  focusing quality of each modulation we will use the intensity at the central pixel, rather than the total intensity throughout the  sensor. 
% \BE
% \Mtric_{Conf}(\bu)=I(0).
% \EE
%$\OpPr_{\text{sens}}$ 

Denoting by $\Fr_{0,\rightarrow}$ the central row of the Fourier transformation from the SLM plane to the image plane, and using the notations of \secref{sec:problem_formulation},
the contribution of the particle $\ptd_k$ to our measurement at the central pixel is
\BE\label{eq:ctrl-pixel}\Fr_{0,\rightarrow} \DiagM(\boutu)\ckTMo.\EE
Assuming w.l.o.g., that the central pixel is measuring the DC component of the Fourier transformation, we can express the value at the central pixel  in \equref{eq:ctrl-pixel} as the product of the SLM modulation $\boutu$ at the imaging arm, with the corresponding column of the outgoing transmission matrix:
\BE\Fr_{0,\rightarrow} \DiagM(\boutu)\ckTMo = {\boutu}^\top \ckTMo.\EE

By modulating both illumination and imaging arms,  we can express the energy of the central pixel  as: 
\BEA\label{eq:inc-confocal} \vspace{-0.1cm}
\!\Mtric_{\text{Conf}}(\binu,\boutu)\!&\!\equiv\!&\! I(0)
=\sum_k |{\boutu}^{\top} \ckTMo|^2 |\rkTMi \binu|^2\nonumber\\\!&\!=\!&\! \sum_k |\boutou_k|^2\cdot  |\binou_k|^2.
\EEA
%\BE
%\begin{gathered}
%\Mtric_{\text{Conf}}(\binu,\boutu)\equiv I(0)=\\
%\sum_k |{\boutu}^{\top} \ckTMo|^2 |\rkTMi \binu|^2= \sum_k |\boutou_k|^2\cdot  |\binou_k|^2.
%\end{gathered}
%\vspace{-0.1cm}
%\EE
with $\binou=\TMi \binu$ and $\boutou=\boutu^T \TMo$.

As mentioned in \equref{eq:bounded-v}, the energy of $\binou$ is bounded, and due to reciprocity the same applies for $\boutou$. 
It is easy to see that this score is maximized when $\binou,\boutou$ are both one-hot vectors at the same entry $k$. That is, the score of \equref{eq:inc-confocal} is maximized when the excitation modulation $\binu$ brings all light to one of the particles $\ptd_k$, and the modulation at the imaging arm $\boutu$ corrects the wavefront emitted from the same particle $\ptd_k$ and brings all of it into the central pixel. 


%As before, this score favors one-hot $\bou$ vectors and the score is maximized when all light is focused at a single spot. 

In particular, if the excitation and emission wavelengths are sufficiently similar so that we can approximate $\TMo \approx {\TMi}^\top$, it is best to use the same modulation at both illumination and imaging arms, and the score of \equref{eq:inc-confocal} reduces to $\sum_k |\bou_k|^4$ as in the variance-maximization and two-photon cases.

While the confocal score is equivalent to the variance maximization score above, it is significantly less susceptible to noise. This is due to the fact that the small number of photons we have at hand are collected at a single spot, rather than being spread over multiple pixels.  \figref{fig:data_type}(c-d) shows the images emitted from a single neural spot with and without modulation in the imaging arm, and the significant noise reduction. 


 

\input{fig_setup}
In this work we have  explicitly optimized the confocal score (\equref{eq:inc-confocal}) using standard Hadamard basis optimization~\cite{PopoffPhysRevLett2010}, detailed in the supplement. In our case the excitation and emission wavelengths are similar, yet not identical. We start the optimization by restricting the modulation on both arms to be equivalent. Once this optimization has converged, we use it as an initialization for a second, refined optimization, which seeks an independent modulation for each wavelength. 
Overall the Hadamard optimization is significantly slower than~\cite{Dror22}. 
We note that when all fluorescent sources $\ptd_k$ have the same power, there are $K$ different solutions that can maximize  \equref{eq:inc-confocal} and an optimization may converge to any of them.
Also note that we constrain the solution such that regardless of the position of $\ptd_k$, it will be imaged in the central pixel. If  $\ptd_k$ is not at the center of the frame, the wavefront $\boutou$, placed at the Fourier plane of the imaging system, will contain a tilt shifting $\ptd_k$ to the central pixel.

 \boldstart{Iterative phase conjugation:}
Recently~\cite{Dror22} has proposed an incoherent iterative phase conjugation algorithm that can rapidly estimate a wavefront shaping modulation. This algorithm is not explicitly maximizing a cost function. It uses fast power iteration to seek an excitation wavefront which is an eigenvector of the transmission matrix of the tissue, although  the definition of transmission matrices with incoherent light is a bit challenging. Intuitively, when using the same modulation in both arms, the confocal cost of \equref{eq:inc-confocal} is maximized when the  wavefront $\ckTMo$ emerging from the system is correlated with the illuminating wavefront  $\bu$. This means that the optimum can also be thought of as an eigenvector. 
The algorithm of~\cite{Dror22} was successfully applied on fluorescent beads, which are both strong and sparse.
In this work we apply the confocal score of \equref{eq:inc-confocal} to real biological data such as EGFP neurons. This data is significantly weaker, and also the fluorescent target exhibits a continuous area rather than sparse isolated dots. 
The algorithm of~\cite{Dror22} heavily relies on the existence of some speckle variation  in the input image due to the need to retrieve the phase of the wavefront arriving the sensor from the measured intensity. Thus, it does not directly apply to continuous  fluorescent sources, where not much speckle variation can be measured. 




==> tex_files/optimization.tex <==
\section{Optimization}
\label{sec:optim}

	\subfile{./fig_converging}
	
	
	
	

	
	
	
	

==> tex_files/problem_formulation_long.tex <==

\section{Problem formulation} \label{sec:problem_formulation}


\boldstart{Imaging setup:}
Consider the schematic of \figref{fig:setup_simp_1}. A laser beam illuminates a tissue sample, and an SLM can modulate its shape.  
The illumination wavefront propagates through the scattering tissue and excites the fluorescent target behind it. We wish to image that target, but the emitted light is scattered again through the tissue on its way to the camera.  A second phase SLM at the  imaging arm modulates the emitted light. Lastly, the modulated light is measured by the front main camera.
While  omitted from the simplified schematic,  our SLMs  are placed at the Fourier planes of the system.



The setup includes a second validation camera behind the tissue sample %, which is used 
to assess focusing quality and  capture a clean reference image of the same target.
While earlier research demonstrations of wavefront-shaping use this camera to provide feedback to the algorithm, we emphasize that our goal in this research is to develop non-invasive techniques that can only use feedback by the main (front)  camera. The validation camera {\em does not} provide any input to the algorithm.

While some  research on wavefront shaping and adaptive optics modulates only the illumination or imaging arms, our problem formulation below will consider modulations at both arms. 


% In \figref{fig:setup} we visualize a wavefront-shaping imaging setup.  A laser beam illuminates a tissue sample via  a microscope objective. A phase SLM at the Fourier plane of the illumination arm modulates the illumination pattern.
%We wish to image a target at the back of the tissue layer. This can either be a reflective/scattering target, or a fluorescent one as we describe next. 
%  The light returning from the target is collected via the same objective, and reflected at a  beam-splitter. A second phase SLM at the Fourier plane of the imaging arm modulates the emitted light. Lastly, the modulated light is measured by the front main camera, which captures the images used by our algorithm. We note that we chose to place the SLMs in  Fourier planes mostly for the simplicity of exposition, but in practice there are benefits to placing them at other places in the optical system~\cite{Mertz:15}. 
%  %We used a $10$nm bandpass filter on the emission light so that the recorded intensity is sufficiently monochromatic and speckles are visible. 
%In our setup we include a second validation camera behind the tissue sample. 
%While earlier research on wavefront-shaping use this camera to provide feedback to the algorithm, we emphasize that our goal in this research is to develop non-invasive algorithms that can only use feedback by the main (front)  camera. Measurements from the validation camera are \emph{not} used by our algorithm. However, such a camera can help assess focusing quality and  image an undistorted reference of the target.
%We note that some of the research on wavefront shaping and adaptive optics modulated only the illumination or imaging arms.  For generality, our problem formulation below will consider modulations at both arms. 

% \vspace{-0.1cm}
\boldstart{Image formation model:} 
Consider a set of $K$ fluorescent particles inside a  sample, and denote their positions by $\ptd_1,\ldots,\ptd_K$.
We assume the SLM in the illumination arm is illuminated with a spatially uniform plane wave and use the SLM to display a complex 2D electric field that we denote by  $\bu$.  Although $\bu$ is a 2D field, we reshape it as a 1D vector. We also use $\bou$ to denote a $K\times 1$ vector of  the field propagating through the sample at each of the $K$  fluorescent sources. 

 
 The relation between $\bu$ and $\bou$ is linear and can be described as a  multiplication by a (very large)  matrix  $\bou=\TMi \bu$, where  $\TMi$ is the incoming transmission matrix, describing the forward coherent light propagation in the tissue. We note that $\TMi$   is specific to the tissue sample being tested, and different tissue samples are described by very different transmission matrices. For thick tissue, $\TMi$ can be an arbitrarily complex matrix incorporating multiple scattering events in the tissue.
Likewise, if the light returning from the target is coherent, its propagation  to the SLM of the imaging arm can be described as $\TMo\bou$, where $\TMo$ is the coherent back-propagation transmission matrix.

%
%The propagation of light from the illumination SLM plane to the particles and back to the SLM of the imaging arm 
%is then modeled using the \emph{combined transmission matrix}  \vspace{-0.2cm}\BE \label{eq:Ta-def} \TMa\equiv\TMo\cdot \TMi. \vspace{-0.2cm}\EE 

We denote by $\CamSLMVect$ the wavefront placed on the SLM of the imaging arm, and by $\DiagM(\CamSLMVect)$ a diagonal matrix with  $\CamSLMVect$ on its diagonal. Our SLMs are placed at the Fourier planes of the imaging system, and we denote by $\Fr$ the Fourier transform of the wavefront from the SLM to the camera sensor. With this notation, coherent light propagating from the target particles to the sensor, through the SLM, can be expressed as
\BE
\Fr \DiagM(\CamSLMVect)\TMo\bou.
\EE
 %, so that the sensor measures $\OpPr_{\text{sens}}\TMa \bu$. 
%Assuming w.l.o.g that the SLM is placed at the Fourier plane of the imaging arm, $\OpPr_{\text{sens}}$ is just a Fourier transform.

In the fluorescent case, the emissions from different points are incoherent, hence the recorded intensity is the sum of emitted intensity from each fluorescent bead:
%In the fluorescent case,  the emissions from different points are incoherent.
%%, and the fluorescent emission is proportional to the intensity of $|\bou|^2$ rather than to the complex field  $\bou$ itself. 
% The recorded intensity can be expressed as \vspace{-0.2cm}
\BE \label{eq:img-form-incoherent} 
I=\sum_k |\Fr \DiagM(\CamSLMVect)\ckTMo|^2 |\bou_{{k}}|^{2\alpha}, \vspace{-0.12cm}
\EE
%
%\Dror{I think we can form the equation much simpler. this is very complicated. I suggest:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We denote by $\bw$ the wavefront placed on the SLM of the imaging arm, and by $\bW$ a diagonal matrix with  $\bw$ on its diagonal. We denote by $\Fr\{\cdot\}$ a Fourier transform, describing wavefront propagation from the SLM plane to the camera sensor plane. %, so that the sensor measures $\OpPr_{\text{sens}}\TMa \bu$. 
%%Assuming w.l.o.g that the SLM is placed at the Fourier plane of the imaging arm, $\OpPr_{\text{sens}}$ is just a Fourier transform.
%
%
%In the fluorescent case,  the emissions from different points are incoherent.
%%, and the fluorescent emission is proportional to the intensity of $|\bou|^2$ rather than to the complex field  $\bou$ itself. 
%The recorded intensity can be expressed as \vspace{-0.2cm}
%\BE \label{eq:img-form-incoherent-dror} 
%I=\sum_k |\Fr\{ \bW\ckTMo\}|^2 |\bou_{{k}}|^{2\alpha}, \vspace{-0.12cm}
%\EE
%\Dror{until here}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where  $|\bou_{{k}}|^2$ is the energy of the excitation light arriving at particle $\ptd_k$, and $\ckTMo$ is the $k$-th column of $\TMo$, so that $\Fr \DiagM(\CamSLMVect) \ckTMo$ is the wavefront arriving to the sensor from  $\ptd_k$.  
%Since light emitted from a fluorescent particle is incoherent with the light emitted from other particles, effectively the sensor sums the intensity of the wavefronts emitted by different particles, and their phases do not interfere. 
In \equref{eq:img-form-incoherent} $\alpha$ denotes the type of fluorescent excitation. The simplest case  $\alpha=1$ is known as single-photon fluorescence where the emission is linear in the excitation energy $|\bou_{{k}}|^{2}$. In two-photon fluorescence,  $\alpha=2$, namely the emission is proportional to the squared excitation. 
%Working with linear fluorescence is significantly simpler and cheaper, but as we explain below, a non-linear (two-photon) fluorescence feedback simplifies modulation estimation. 


 
 \boldstart{Phase conjugation: }
When the incoming and outgoing light have the same wavelength, the Helmholtz  reciprocity principle leads to wave conjugation. Namely, if we record the wavefront emitted from a source point inside the tissue and illuminate with the conjugate wavefront,  light will focus at the same point.  This implies that the returning transmission matrix is the transpose of the incoming one ~\cite{RevModPhys.89.015005}:  \vspace{-0.2cm}\BE \label{eq:conj-transmission-M} \TMo={\TMi}^\top. \vspace{-0.2cm}\EE %\Dror{I uncommented this note: Note that this is just a transpose and not the Hermitian (conjugate) transpose.}
In the fluorescent case,  $\TMi,\TMo$ describe propagation at two different excitation and emission wavelengths. However, for linear single-photon fluorescence the excitation and emission wavelengths are relatively similar and 
   $\TMo\approx {\TMi}^\top$. While our algorithm {\em does not} require the incoming and outgoing transmission matrices to be the same, this similarity will help us draw intuition on what is being optimized.
 
%   
%
%
%In particular, in the adaptive optics literature,  one often attempts to correct aberrations caused by imperfect optics and not by the tissue (\figref{fig:aberration_types}(a)). This implies that the {\em same} correction  can be used over a large image region. 
%At the other extreme, wavefront shaping algorithms aim to correct aberrations caused by a thick  tissue exhibiting volumetric scattering. Wavefront shaping is a significantly harder task, first because it attempts to recover  larger aberrations, and often the speckle pattern emerging from a single aberrated point  spreads over a very wide sensor area. The more serious challenge, however,  results from the fact that for thick tissue, memory effect correlations are small~\cite{osnabrugge2017generalized,SeeThroughSubmission}, and the rows of the transmission matrices are very different from each other, and we would need {\em a different modulation for every pixel we aim to image}.
%
%


\boldstart{Normalization:}
we assume for simplicity that our transmission matrices are normalized such that every column or row has a unit energy, that is for every $k$ \vspace{-0.1cm}
\BE\label{eq:bounded-rows}
\sum_x |\TMo_{x,k}|^2= 1,\quad \sum_x |\TMi_{k,x}|^2=1. \vspace{-0.1cm}
\EE
This means that the total amount of energy that can arrive to particle $\ptd_k$ or emerge from it is fixed.
As the laser energy is fixed, we also assume w.l.o.g. that all illumination vectors have a unit norm $\|\bu\|=1$.
As propagation through the tissue does not generate new energy,  every incoming vector $\bu$ should satisfy  \vspace{-0.1cm}
$\|\TMi \bu\|\leq1$ and thus the energy at the target is also bounded \BE \label{eq:bounded-v} \sum_k |\bou_k|^2\leq 1.\EE
